Structural Reasoning Improves Molecular Understanding of LLM

Recently, large language models (LLMs) have shown significant progress, approaching human perception levels. In this work, we demonstrate that despite these advances, LLMs still struggle to reason using molecular structural information. This gap is critical because many molecular properties, including functional groups, depend heavily on such structural details. To address this limitation, we propose an approach that sketches molecular structures for reasoning. Specifically, we introduce Molecular Structural Reasoning (MSR) framework to enhance the understanding of LLMs by explicitly incorporating the key structural features. We present two frameworks for scenarios where the target molecule is known or unknown. We verify that our MSR improves molecular understanding through extensive experiments.

==> figure/1.failure_case.tex <==
\begin{figure}[t]
% \vspace{-0.1in}
    \centering
    \includegraphics[width=\linewidth]{figure/failure_case.pdf}
    \caption{\textbf{The failure case of GPT-4o for the inference of structural information given the molecular SMILES.} The \textcolor{red}{red} color indicates the wrong generated structural information while the \textcolor{grn}{green} color indicates the correct answer. Note that we visualize the molecular graph for illustration purposes; GPT-4o does not take them as inputs.}\label{fig: failure_case}
    \vspace{-0.1in}
\end{figure}

==> figure/2.analysis.tex <==
\begin{figure}[t]

    \centering
    \includegraphics[width=0.98\linewidth]{figure/analysis.pdf} 
    \vspace{-0.1in}
    \caption{\textbf{Analysis of LLMs' Understanding of Structural Information.} Green and blue colors represent LLaMA3-8B and GPT-4, respectively. Patterns denote the input types: crossed patterns represent SMILES representations (\textit{Mol2Structure}), and diagonally crossed patterns represent the text descriptions (\textit{Text2Structure}).
    }\label{fig: analysis}
    \vspace{-0.3in}
\end{figure}

==> figure/2.analysis_prompt.tex <==
\begin{figure}[t]
% \vspace{-0.1in}
    \centering
    \includegraphics[width=0.98\linewidth,height=2in]{example-image-a} 
    \caption{\textbf{Example prompts for molecule captioning and text-based molecule generation.}}\label{fig: analysis_prompt}
    \vspace{-0.1in}
\end{figure}

==> figure/4.iteration.tex <==
\begin{figure}[t]
% \vspace{-0.1in}
    \centering
    \includegraphics[width=0.98\linewidth, height=5cm]{example-image-a}
    \caption{\textbf{An example of iterative alignment between CoT and output.}
    }\label{fig: iterative}
    % \vspace{-0.1in}
\end{figure}


==> figure/4.ring_decomp.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
\centering
\vspace{-0.1in}
\includegraphics[width=\linewidth]{figure/ring_decomp.pdf}
% \begin{subfigure}[b]{\linewidth}
%     \includegraphics[width=\linewidth]{figure/ring_wo_decomp.pdf}
%     % \vspace{-0.2in}
%     \caption{Ring decomposiiton in ring compound CoT.} \label{fig: ring}
%     \vspace{-0.2in}
% \end{subfigure}
% \begin{subfigure}[b]{\linewidth}
%         \includegraphics[width=\linewidth]{figure/ring_with_decomp.pdf}
%     % \vspace{-0.2in}
%     \caption{Ring decomposiiton in ring compound CoT.} \label{fig: ring}
%     \vspace{-0.2in}
% \end{subfigure}
\caption{\textbf{The ring decomposition process for ring compound CoT.}\label{fig: ring}}
\end{wrapfigure}

==> table/tab_chemcrow.tex <==
\begin{table}
  \caption{\textbf{Comparison to ChemCrow.} The left part shows the molecule captioning results and the right part shows the text-based molecule generation results. }\label{tab:chemcrow}
  \vspace{-0.1in}
  \centering
  \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccccccc}
    \toprule[1.25pt]
    & \multicolumn{3}{c}{\textbf{Molecule captioning}} & \multicolumn{6}{c}{\textbf{Text-based molecule generation}} \\
    % \midrule
   \cmidrule(lr){2-4} \cmidrule(lr){5-10} 
    & \textbf{BLEU2}  &  \textbf{ROUGE2}  & \textbf{METEOR} & \textbf{BLEU} & \textbf{Exact} & \textbf{Leven.} $\downarrow$ &  \textbf{Morgan} & \textbf{FCD} $\downarrow$ & \textbf{Validity} \\
    \midrule[1.25pt]
    GPT-4o & 0.232  & 0.183 &  0.291 & {0.521} & 0.079 & {40.87} & {0.583} & 3.67 & {0.881}  \\
    ChemCrow (GPT-4o) & 0.162 & 0.097  & 0.225 & 0.306 & 0.194 & 56.46  & 0.555 & 2.31 & 0.851   \\
  % Ours (GPT-4o) & 0.286 & 0.199  & 0.341 & 0.509 & 41.68 & 0.783  & 0.571 & 1.57 & 0.846  \\
    Ours (ChemT5-base) & 0.639 & 0.553 & 0.657 & 0.878 & 0.421 & 12.76 & 0.804 & 0.26 & 0.982\\
  
    \bottomrule[1.25pt]
    \end{tabular}}
    \vspace{-0.2in}
\end{table}


==> table/tab_gen_mol2text.tex <==
\begin{table}
  \caption{\textbf{Generalist Performance.} The left part shows the molecule captioning results and the right part shows the text-based molecule generation results. }\label{tab:generalist}
  % \vspace{-0.1in}
  \centering
  \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccc|ccccccccc}
    \toprule[1.25pt]
    & BL.-2 & BL.-4 & ROU.-1 & ROU.-2 & ROU.-4 & METEOR & BLEU & Exact & Leven. $\downarrow$ & MACCS & RDK & Morgan & FCD $\downarrow$ & Valid. \\
    \midrule[1.25pt]
    Llama3 & 0.211 & 0.117 & 0.367 & 0.183 & 0.308 & 0.257 & 0.251 & 0.007 & 117.30 & 0.586 & 0.352 & 0.276 & 13.11 & 0.629   \\
    \quad +\Algname & 0.\textbf{259} & \textbf{0.158} & \textbf{0.401} & \textbf{0.208} & \textbf{0.324} & \textbf{0.341} & \textbf{0.259} & \textbf{0.008} & \textbf{109.77} & 0.579 & 0.279 & \textbf{0.344} & \textbf{4.47} & \textbf{0.669} \\
    \midrule
    GPT-4o & 0.232 & 0.128 & 0.389 & 0.183 & 0.307 & 0.291 & \textbf{0.521} & 0.079 & \textbf{40.87} & \textbf{0.797} & 0.496 & \textbf{0.583} & 3.67 & \textbf{0.881} \\ 
    \quad +\Algname & \textbf{0.286} & \textbf{0.174} & \textbf{0.405} & \textbf{0.199} & \textbf{0.313} & \textbf{0.341} & 0.509  & \textbf{0.088} & 41.68 & 0.783 & \textbf{0.498} & 0.571  & \textbf{1.57} &   0.846  \\
    \bottomrule[1.25pt]
    \end{tabular}}
    
\end{table}

==> table/tab_gen_text2mol.tex <==
\definecolor{whitegray}{RGB}{243, 243, 243} 


\begin{table}
  \caption{\textbf{Text-based molecule generation performance.} The \textcolor{teal}{teal} color indicates the improvement while the \textcolor{red}{red} color indicates the reduction.}\label{tab:text2mol}
  \vspace{-0.1in}
  \centering
  \resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccccccccc}
    \toprule[1.25pt]
      & \multicolumn{2}{c}{\textbf{BLEU} } & \multicolumn{2}{c}{\textbf{Exact} } &\multicolumn{2}{c}{\textbf{Levenshtein} $\downarrow$} &\multicolumn{2}{c}{\textbf{MACCS FTS}} &\multicolumn{2}{c}{\textbf{RDK FTS}} &\multicolumn{2}{c}{\textbf{Morgan FTS}} &\multicolumn{2}{c}{\textbf{FCD}$\downarrow$} &\multicolumn{2}{c}{\textbf{Validity}}\\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}
     Models  & Met. & $\mathbf{\Delta}$ & Met. &  $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ \\
    \midrule[1.25pt]
    % \rowcolor{whitegray} \multicolumn{17}{l}{\textit{Generalists (10-shot learning)}} \\
    \midrule
    
    Llama3  & 0.251 & - & 0.007 & - & 117.30 & - & 0.586 & - & 0.352 & - & 0.276 & - & 13.11 & - & 0.629 & - \\
    \quad +\Algname & 0.259 & \textcolor{teal}{0.008} & 0.008 & \textcolor{teal}{0.001} & 109.77 & \textcolor{teal}{7.53} & 0.579 & \textcolor{red}{0.007} & 0.279 & \textcolor{red}{0.073} & 0.344 & \textcolor{teal}{0.068} & 4.47 & \textcolor{teal}{8.64} & 0.669 & \textcolor{teal}{0.040}  \\
    \midrule
    GPT-4o & 0.521 & - & 0.079 & - & 40.87 & - & 0.797 & - & 0.496 & - & 0.583 & - & 3.67 & - & 0.881 & - \\
    \quad +\Algname & 0.509 & \textcolor{red}{0.012} & 0.088 & \textcolor{teal}{0.009} & 41.68 & \textcolor{teal}{0.081} & 0.783 & \textcolor{red}{0.014} & 0.498 & \textcolor{teal}{0.002} & 0.571 & \textcolor{red}{0.012} & 1.57 & \textcolor{teal}{2.10} & 0.846 & \textcolor{red}{0.035} \\
    \bottomrule[1.25pt]
    \end{tabular}
    }
    \vspace{-0.2in}
\end{table}

==> table/tab_iter.tex <==
\setlength\intextsep{0pt}
\begin{wraptable}{R}{0.5\textwidth}
\vspace{-0.02in}
  \caption{\textbf{Effectiveness of iterative CoT alignment.}} \label{tab: iter}
  \vspace{-0.1in}
  \centering
  \scalebox{0.8}{
    \begin{tabular}{lccc}
    \toprule
    Dataset & Vocab. size & Rep. size & $N^2$ \\
    \midrule
    % Ego-small & 225 & 83 & 289 \\
    % Com.-small & 64 & 80 & 400  \\
    Planar & 676 & 181 & 4096 \\
    Lobster & 2401 & 99 & 9604 \\ 
    Enzymes & 361 & 149 & 15625 \\
    SBM & 12321 & 1129 & 34969 \\
    Ego & 58081 & 1071 & $>10^{6}$ \\
    Grid & 361 & 684 & 467856 \\
    Proteins & 62500 & 1575 & $>10^{6}$ \\
    3D point cloud & 111556 & 10886 & $>10^{7}$ \\
    \bottomrule
  \end{tabular}
  }
%  \vspace{-0.2in}
\end{wraptable}


==> table/tab_mol2text_lm_old.tex <==
\definecolor{whitegray}{RGB}{243, 243, 243} 

\begin{table}[t]
  \caption{\textbf{Molecule Captioning Performance for L+M dataset.} $\Delta$ denotes the performance difference between the original model and the one incorporated with \Algname. The \textcolor{teal}{teal} color indicates the improvement.}\label{tab:mol2text_lm}
  % \vspace{-0.1in}
  \centering
  \resizebox{\linewidth}{!}{
\begin{tabular}{cccccccccccccc}
    \toprule[1.25pt]
      & \multicolumn{2}{c}{\textbf{BLEU-2} } & \multicolumn{2}{c}{\textbf{BLEU-4} } &\multicolumn{2}{c}{\textbf{ROUGE-1} } &\multicolumn{2}{c}{\textbf{ROUGE-2} } &\multicolumn{2}{c}{\textbf{ROUGE-L} } &\multicolumn{2}{c}{\textbf{METEOR} } \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
     Models & Metric & $\mathbf{\Delta}$ & Metric &  $\mathbf{\Delta}$ & Metric & $\mathbf{\Delta}$ & Metric & $\mathbf{\Delta}$ & Metric & $\mathbf{\Delta}$ & Metric & $\mathbf{\Delta}$ \\
    \midrule[1.5pt]
    MolT5-small & 0.709 & - & 0.512 & - & 0.745 & - & 0.558 & - & 0.544 & - & 0.701 & - \\
    \quad+\Algname  \\
    \midrule
    MolT5-base & 0.738 & - & 0.535 & - & 0.750 & - & 0.559 & - & 0.539 & - & 0.718 & -  \\
    \quad+\Algname &  & \textcolor{teal}{0.} & 0. & \textcolor{teal}{0.} & 0. &\textcolor{teal}{0.}& 0. &\textcolor{teal}{0.}& 0. &\textcolor{teal}{0.}& 0. &\textcolor{teal}{0.} \\
    \midrule
    MolT5-large & 0.769 & - & 0.556 & - & 0.777 & - & 0.580 & - & 0.557 & - & 0.743 & - \\
    \quad +\Algname  & \textbf{0.} & \textcolor{teal}{0.} & \textbf{0.} & \textcolor{teal}{0.} & \textbf{0.} & \textcolor{teal}{0.} & \textbf{0.} & \textcolor{teal}{0.} & \textbf{0.} & \textcolor{teal}{0.} & \textbf{0.} &\textcolor{teal}{0.} \\
    \bottomrule[1.25pt]
    \end{tabular}
    }
    \vspace{-0.15in}
\end{table}

==> table/tab_mol2text_old.tex <==
\definecolor{whitegray}{RGB}{243, 243, 243} 

\begin{table*}[t]
  \caption{\textbf{Molecule Captioning Performance for ChEBI-20 dataset.} $\Delta$ denotes the performance difference between the original model and the one incorporated with \Algname. The \textcolor{teal}{teal} color indicates the improvement.}\label{tab:mol2text}
  % \vspace{-0.1in}
  \centering
  \resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccccc}
    \toprule[1.25pt]
      & \multicolumn{2}{c}{\textbf{BLEU-2} } & \multicolumn{2}{c}{\textbf{BLEU-4} } &\multicolumn{2}{c}{\textbf{ROUGE-1} } &\multicolumn{2}{c}{\textbf{ROUGE-2} } &\multicolumn{2}{c}{\textbf{ROUGE-L} } &\multicolumn{2}{c}{\textbf{METEOR} } \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
     Models & Metric & $\mathbf{\Delta}$ & Metric &  $\mathbf{\Delta}$ & Metric & $\mathbf{\Delta}$ & Metric & $\mathbf{\Delta}$ & Metric & $\mathbf{\Delta}$ & Metric & $\mathbf{\Delta}$ \\
    % \midrule[1.25pt]
    % \rowcolor{whitegray} \multicolumn{13}{l}{\textit{Baselines (without CoTs)}} \\
    % \midrule
    % RNN & 0.251 & - & 0.176 & - &0.450 & - &0.278 & - & 0.394 & - & 0.363 & - \\
    % \midrule
    % T5-base & 0.511 & - & 0.423 & - & 0.607 & - & 0.451 & - & 0.550 & - & 0.539 & - \\
    % \midrule
    % Transformer & 0.061 & - & 0.027 & - & 0.204 & - & 0.087 & - & 0.186 & - & 0.114 & - \\
    % \midrule
    % MolXPT & 0.594 & - & 0.505 & - & 0.660 & - & 0.511 & - & 0.597 & - & 0.626 & - \\
    % \midrule
    BioT5 & 0.635 & - & 0.556 & - & 0.692 & - & 0.559 & - & 0.633 & - & 0.656 & - \\
    \midrule[1.5pt]
    \rowcolor{whitegray} \multicolumn{13}{l}{\textit{Specialists (fine-tuning)}} \\
    % \midrule
    % MolT5-small & 0.519 & - & 0.436 & - & 0.620 & - & 0.469 & - & 0.563 & - & 0.551\\
    % \quad +\Algname \\
    \midrule
    MolT5-base & 0.540 & - & 0.457 & - & 0.634 & - & 0.485 & - & 0.578 & - & 0.569 & -  \\
    % \quad +\Algname (epoch 220) & 252M & 0.578 & \textcolor{teal}{+7.0\%} & 0.486 &  \textcolor{teal}{+6.3\%} & 0.648 &  \textcolor{teal}{+2.2\%} & 0.495 & \textcolor{teal}{+2.1\%} & 0.588 & \textcolor{teal}{+1.7\%} & 0.603 & \textcolor{teal}{+6.0\%} \\
    \quad+\Algname & 0.592 & \textcolor{teal}{0.052} & 0.507 & \textcolor{teal}{0.050} & 0.667 &\textcolor{teal}{0.043}& 0.523 &\textcolor{teal}{0.038}& 0.606 &\textcolor{teal}{0.028}& 0.619 &\textcolor{teal}{0.050} \\
    % \quad +\Algname (epoch 220) & 0.578 & \textcolor{teal}{0.038} & 0.486 &  \textcolor{teal}{0.029} & 0.648 &  \textcolor{teal}{0.014} & 0.495 & \textcolor{teal}{0.010} & 0.588 & \textcolor{teal}{0.010} & 0.603 & \textcolor{teal}{0.034} \\
    \midrule
    MolT5-large & 0.594 & - & 0.508 & - & 0.654 & - & 0.510 & - & 0.594 & - & 0.614 & - \\
    \quad +\Algname  & \textbf{0.645} & \textcolor{teal}{0.051} & \textbf{0.567} & \textcolor{teal}{0.059} & \textbf{0.699} & \textcolor{teal}{0.045} & \textbf{0.568} & \textcolor{teal}{0.058} & \textbf{0.639} & \textcolor{teal}{0.045} & \textbf{0.666} &\textcolor{teal}{0.052} \\
    % \quad +\Algname (epoch 110)  & 0.610 & \textcolor{teal}{0.016} & 0.523 & \textcolor{teal}{0.015} & 0.669 & \textcolor{teal}{0.015} & 0.525 & \textcolor{teal}{0.015} & 0.609 & \textcolor{teal}{0.015} & 0.632 &\textcolor{teal}{0.018} \\
    \midrule
    ChemT5-small & 0.553 & - & 0.462 & - & 0.633 & - & 0.481 & - & 0.574 & - & 0.583 & -  \\
    \quad +\Algname & 0.601 & \textcolor{teal}{0.048} & 0.513 & \textcolor{teal}{0.050} & 0.664 & \textcolor{teal}{0.031} & 0.519 & \textcolor{teal}{0.038} & 0.603 & \textcolor{teal}{0.029} & 0.624 &\textcolor{teal}{0.042} \\
    \midrule
    ChemT5-base & 0.580 & - & 0.490 & - & 0.647 & - & 0.498 & - & 0.586 & - & 0.604 \\
    \quad +\Algname & 0.639 & \textcolor{teal}{0.059} &0.560 &\textcolor{teal}{0.070}& 0.687 &\textcolor{teal}{0.040}& 0.553 &\textcolor{teal}{0.055}& 0.626 &\textcolor{teal}{0.040}& 0.657 &\textcolor{teal}{0.053} \\
    \midrule[1.25pt]
    \rowcolor{whitegray} \multicolumn{13}{l}{\textit{Generalists (without fine-tuning)}} \\
    \midrule
    Llama3 & 0.211 & - & 0.117 & - & 0.367 & - & 0.183 & - & 0.308 & - & 0.257 & -  \\
    \quad +\Algname & 0.259 &\textcolor{teal}{0.048}& 0.158 &\textcolor{teal}{0.041}& 0.401 &\textcolor{teal}{0.034}& 0.208 &\textcolor{teal}{0.025}& 0.324 &\textcolor{teal}{0.016}& 0.341 & \textcolor{teal}{0.084} \\
    \midrule
    GPT-4o & 0.232 & - & 0.128 & - & 0.389 & - & 0.183 & - & 0.307 & - & 0.291 & - \\ 
    \quad +\Algname & 0.286 &\textcolor{teal}{0.054}& 0.174 &\textcolor{teal}{0.046}& 0.405 &\textcolor{teal}{0.016}& 0.199 &\textcolor{teal}{0.016}& 0.313 &\textcolor{teal}{0.006}& 0.341 &\textcolor{teal}{0.050}\\
    \midrule
    \textcolor{black}{Mol-Instructions} & 0.217 & - & 0.143 & - & 0.337 & - & 0.196 & - & 0.291 & - & 0.254 & - \\
    \textcolor{black}{\quad +\Algname} & 0.347 & \textcolor{teal}{0.130} & 0.275  &  \textcolor{teal}{0.132} & 0.601 &  \textcolor{teal}{0.264} & 0.518 &  \textcolor{teal}{0.322} & 0.593 &  \textcolor{teal}{0.302} & 0.520 &  \textcolor{teal}{0.266} \\
    \bottomrule[1.25pt]
    \end{tabular}
    }
    \vspace{-0.15in}
\end{table*}

==> table/tab_text2mol_new.tex <==
\definecolor{whitegray}{RGB}{243, 243, 243} 


\begin{table}
% \vspace{-0.2in}
  \caption{\textbf{Text-based molecule generation performance.} The \textcolor{teal}{teal} color indicates the improvement while the \textcolor{red}{red} color indicates the reduction.}\label{tab:text2mol_new}
  
  \centering
  \resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccc}
    \toprule[1.25pt]
& BLEU & Exact & Levenshtein $\downarrow$ & MACCS FTS & RDK FTS & Morgan FTS & FCD $\downarrow$ & Validity \\
    % athbf{\Delta}$ & Met. &  $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ \\
    \midrule[1.25pt]
    \rowcolor{whitegray} \multicolumn{9}{l}{\textit{Baselines (without CoTs)}} \\
    \midrule
    RNN & 0.652 & 0.005 & 38.09 & 0.591 & 0.400 & 0.362 & 4.55 & 0.542 \\
    \midrule
    Transformer & 0.499 & 0.000 & 57.66 & 0.480 & 0.320 & 0.217 & 11.32 & 0.906 \\
    \midrule
    T5-base & 0.762 & 0.069 & 24.95 & 0.731 & 0.605 & 0.545 & 2.48 & 0.660 \\
    \midrule
    MolXPT & 0.215 &  0.859 & 0.757 & 0.667 & 0.45 & 0.983 \\
    \midrule
    BioT5 & 0.867 & 0.413 & 15.10 & 0.886 & 0.801 & 0.734 & 0.43 & \textbf{1.000} \\
    \midrule[1.5pt]
    \rowcolor{whitegray} \multicolumn{9}{l}{\textit{Specialists (fine-tuning)}} \\
    % % \midrule
    % % MolT5-small & 0.755 & 0.079 & 25.99 & 0.703 & 0.568 & 0.517 & 2.49 & 0.776 \\
    % % \quad+\Algname & 0.860{\tiny\textcolor{teal}{+0.105}& 0.340{\tiny\textcolor{teal}{+0.261}& 14.95{\tiny\textcolor{teal}{+11.04}& 0.908{\tiny\textcolor{teal}{+0.205}& 0.761{\tiny\textcolor{teal}{+0.193}& 0.824{\tiny\textcolor{teal}{+0.307}& 0.31{\tiny\textcolor{teal}{+2.18}& 0.981{\tiny\textcolor{teal}{+0.205} \\
    \midrule
    MolT5-base & 0.769 & 0.081 & 24.46 & 0.721 & 0.588 & 0.529 & 2.18 & 0.772  \\
    \quad+\Algname & 0.863{\tiny\textcolor{teal}{+0.094}} & 0.385{\tiny\textcolor{teal}{+0.304}}& 13.91{\tiny\textcolor{teal}{+10.55}}& 0.918{\tiny\textcolor{teal}{+0.197}}& 0.843{\tiny\textcolor{teal}{+0.255}}& 0.783{\tiny\textcolor{teal}{+0.254}}&
    {\tiny\textcolor{teal}{+}}& 0.983{\tiny\textcolor{teal}{+0.211}}\\
    \midrule
    % % \quad+\Algname & 0.866{\tiny\textcolor{teal}{+0.097} & 0.266{\tiny\textcolor{teal}{+0.185} & 16.522{\tiny\textcolor{teal}{+-7.936} & 0.887{\tiny\textcolor{teal}{+0.166} & 0.786{\tiny\textcolor{teal}{+0.198} & 0.713{\tiny\textcolor{teal}{+0.184} & 0.55{\tiny\textcolor{teal}{+-1.63} & 0.926{\tiny\textcolor{teal}{+0.154} \\
    % \midrule
    MolT5-large & 0.854 & 0.311 & 16.07 & 0.834 & 0.746 & 0.684 & 1.20 & 0.905 \\
    \quad+\Algname \\
    % % \quad+\Algname (epoch 154)  & 0.893{\tiny\textcolor{teal}{+0.039} & 0.381{\tiny\textcolor{teal}{+0.070} & 13.054{\tiny\textcolor{teal}{+-3.017} & 0.906{\tiny\textcolor{teal}{+0.072} & 0.821{\tiny\textcolor{teal}{+0.075} & 0.766{\tiny\textcolor{teal}{+0.082} & 1.96 & \textcolor{red}{0.76} & 0.929{\tiny\textcolor{teal}{+0.024} \\
    \midrule

    ChemT5-small & 0.739 & 0.157 & 28.54 & 0.859 & 0.736 & 0.660 & 0.07 & 0.776 \\
    \quad+\Algname & 0.874{\tiny\textcolor{teal}{+0.135}} & 0.381{\tiny\textcolor{teal}{+0.224}} & 13.22{\tiny\textcolor{teal}{+15.32}}& 0.918{\tiny\textcolor{teal}{+0.059}}& 0.845{\tiny\textcolor{teal}{+0.109}}& 0.787{\tiny\textcolor{teal}{+0.127}}& 0.29+{\tiny\textcolor{red}{0.22}}& 0.976{\tiny\textcolor{teal}{+0.200}} \\
    \midrule
    ChemT5-base & 0.750 & 0.212 & 27.39 & 0.874 & 0.767 & 0.697 & \textbf{0.06} & 0.792 \\
    \quad+\Algname & \textbf{0.878}{\tiny\textcolor{teal}{+0.128}} & \textbf{0.421}{\tiny\textcolor{teal}{+0.209}}& \textbf{12.76}{\tiny\textcolor{teal}{+14.63}}& \textbf{0.924}{\tiny\textcolor{teal}{+0.050}}& \textbf{0.856}{\tiny\textcolor{teal}{+0.089}}& \textbf{0.804}{\tiny\textcolor{teal}{+0.107}}& 0.26+{\tiny\textcolor{red}{0.20}}& 0.982 {\tiny\textcolor{teal}{+0.190}}\\

    % % \midrule
    % % \rowcolor{whitegray} \multicolumn{17}{l}{\textit{Generalists (10-shot learning)}} \\
    % % \midrule
    
    % % Llama3  & 0.251 & 0.007 & 117.30 & 0.586 & 0.352 & 0.276 & 13.11 & 0.629 \\
    % % \quad+\Algname & 0.259{\tiny\textcolor{teal}{+0.008} & 0.008{\tiny\textcolor{teal}{+0.001} & 109.77{\tiny\textcolor{teal}{+7.53} & 0.579 & \textcolor{red}{0.007} & 0.279 & \textcolor{red}{0.073} & 0.344{\tiny\textcolor{teal}{+0.068} & 4.47{\tiny\textcolor{teal}{+8.64} & 0.669{\tiny\textcolor{teal}{+0.040}  \\
    % \midrule
    % GPT-4o & 0.521 & 0.079 & 40.87 & 0.797 & 0.496 & 0.583 & 3.67 & 0.881 \\
    % \quad+\Algname & 0.509 & \textcolor{red}{0.012} & 0.088{\tiny\textcolor{teal}{+0.009} & 41.68{\tiny\textcolor{teal}{+0.081} & 0.783 & \textcolor{red}{0.014} & 0.498{\tiny\textcolor{teal}{+0.002} & 0.571 & \textcolor{red}{0.012} & 1.57{\tiny\textcolor{teal}{+2.10} & 0.846 & \textcolor{red}{0.035} \\
    \bottomrule[1.25pt]
    \end{tabular}
    }
    \vspace{-0.2in}
\end{table}

==> table/tab_text2mol_old.tex <==
\definecolor{whitegray}{RGB}{243, 243, 243} 


\begin{table*}[t]
% \vspace{-0.2in}
  \caption{\textbf{Text-based Molecule Generation Performance for ChEBI-20 dataset.} The \textcolor{teal}{teal} and \textcolor{red}{red} colors indicate the improvement and the reduction, respectively.}\label{tab:text2mol}
  % \vspace{-0.1in}
  \centering
  \resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccccccccc}
    \toprule[1.25pt]
      & \multicolumn{2}{c}{\textbf{BLEU} } & \multicolumn{2}{c}{\textbf{Exact} } &\multicolumn{2}{c}{\textbf{Levenshtein} $\downarrow$} &\multicolumn{2}{c}{\textbf{MACCS FTS}} &\multicolumn{2}{c}{\textbf{RDK FTS}} &\multicolumn{2}{c}{\textbf{Morgan FTS}} &\multicolumn{2}{c}{\textbf{FCD}$\downarrow$} &\multicolumn{2}{c}{\textbf{Validity}}\\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17}
     Models  & Met. & $\mathbf{\Delta}$ & Met. &  $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ & Met. & $\mathbf{\Delta}$ \\
    % \midrule[1.25pt]
    % \rowcolor{whitegray} \multicolumn{17}{l}{\textit{Baselines (without CoTs)}} \\
    % \midrule
    % RNN & 0.652 & - & 0.005 & - & 38.09 & - & 0.591 & - & 0.400 & - & 0.362 & - & 4.55 & - & 0.542 & - \\
    % \midrule
    % Transformer & 0.499 & - & 0.000 & - & 57.66 & - & 0.480 & - & 0.320 & - & 0.217 & - & 11.32 & - & 0.906 & -\\
    % \midrule
    % T5-base & 0.762 & - & 0.069 & - & 24.95 & - & 0.731 & - & 0.605 & - & 0.545 & - & 2.48 & - & 0.660 & - \\
    % \midrule
    % MolXPT & - & - & 0.215 & - & - & - &  0.859 & - & 0.757 & - & 0.667 & - & 0.45 & - & 0.983 \\
    % \midrule
    % BioT5 & 0.867 & - & 0.413 & - & 15.10 & - & 0.886 & - & 0.801 & - & 0.734 & - & 0.43 & - & \textbf{1.000} \\
    \midrule[1.5pt]
    % \rowcolor{whitegray} \multicolumn{17}{l}{\textit{Specialists (fine-tuning)}} \\
    % \midrule
    % MolT5-small & 0.755 & - & 0.079 & - & 25.99 & - & 0.703 & - & 0.568 & - & 0.517 & - & 2.49 & - & 0.776 & - \\
    % \quad +\Algname & 0.860 &\textcolor{teal}{0.105}& 0.340 &\textcolor{teal}{0.261}& 14.95 &\textcolor{teal}{11.04}& 0.908 &\textcolor{teal}{0.205}& 0.761 &\textcolor{teal}{0.193}& 0.824 &\textcolor{teal}{0.307}& 0.31 &\textcolor{teal}{2.18}& 0.981 &\textcolor{teal}{0.205} \\
    % \midrule
    MolT5-base & 0.769 & - & 0.081 & - & 24.46 & - & 0.721 & - & 0.588 & - & 0.529 & - & 2.18 & - & 0.772 & -  \\
    \quad +\Algname & 0.863 & \textcolor{teal}{0.094} & 0.385 &\textcolor{teal}{0.304}& 13.91 &\textcolor{teal}{10.55}& 0.918 &\textcolor{teal}{0.197}& 0.843 &\textcolor{teal}{0.255}& 0.783 &\textcolor{teal}{0.254}& 0.29 &\textcolor{teal}{1.89} & 0.983 &\textcolor{teal}{0.211}\\
    % \quad +\Algname & 0.866 & \textcolor{teal}{0.097} & 0.266 & \textcolor{teal}{0.185} & 16.522 & \textcolor{teal}{-7.936} & 0.887 & \textcolor{teal}{0.166} & 0.786 & \textcolor{teal}{0.198} & 0.713 & \textcolor{teal}{0.184} & 0.55 & \textcolor{teal}{-1.63} & 0.926 &\textcolor{teal}{0.154} \\
    \midrule
    MolT5-large & 0.854 & - & 0.311 & - & 16.07 & - & 0.834 & - & 0.746 & - & 0.684 & - & 1.20 & - & 0.905 & - \\
    \quad +\Algname & \textbf{0.886} &\textcolor{teal}{0.032}& 0.391 &\textcolor{teal}{0.080}& 12.98 &\textcolor{teal}{3.09}& 0.906 &\textcolor{teal}{0.072}& 0.822 &\textcolor{teal}{0.076}& 0.765 &\textcolor{teal}{0.081}& 0.35 &\textcolor{teal}{0.085}& 0.947 & \textcolor{teal}{0.042}\\
    % \quad +\Algname (two) & 0.840 && 0.364 && 15.92 && 0.902 && 0.820 && 0.759 && 0.40 && 0.985 \\
    % \quad +\Algname (epoch 154)  & 0.893 & \textcolor{teal}{0.039} & 0.381 & \textcolor{teal}{0.070} & 13.054 & \textcolor{teal}{-3.017} & 0.906 & \textcolor{teal}{0.072} & 0.821 & \textcolor{teal}{0.075} & 0.766 & \textcolor{teal}{0.082} & 1.96 & \textcolor{red}{0.76} & 0.929 & \textcolor{teal}{0.024} \\
    \midrule

    ChemT5-small & 0.739 & - & 0.157 & - & 28.54 & - & 0.859 & - & 0.736 & - & 0.660 & - & 0.07 & - & 0.776 & - \\
    \quad +\Algname & 0.874 & \textcolor{teal}{0.135} & 0.381 & \textcolor{teal}{0.224} & 13.22 &\textcolor{teal}{15.32}& 0.918 &\textcolor{teal}{0.059}& 0.845 & \textcolor{teal}{0.109}& 0.787 &\textcolor{teal}{0.127}& 0.29 &\textcolor{red}{0.22}& 0.976 & \textcolor{teal}{0.200} \\
    \midrule
    ChemT5-base & 0.750 & - & 0.212 & - & 27.39 & - & 0.874 & - & 0.767 & - & 0.697 & - & \textbf{0.06} & - & 0.792 & - \\
    \quad +\Algname & 0.878 & \textcolor{teal}{0.128} & \textbf{0.421} &\textcolor{teal}{0.209}& \textbf{12.76} &\textcolor{teal}{14.63}& \textbf{0.924 }&\textcolor{teal}{0.050}& \textbf{0.856} &\textcolor{teal}{0.089}& \textbf{0.804} &\textcolor{teal}{0.107}& 0.26 &\textcolor{red}{0.20}& 0.982 &\textcolor{teal}{0.190}\\

    % \midrule
    % \rowcolor{whitegray} \multicolumn{17}{l}{\textit{Generalists (10-shot learning)}} \\
    % \midrule
    
    % Llama3  & 0.251 & - & 0.007 & - & 117.30 & - & 0.586 & - & 0.352 & - & 0.276 & - & 13.11 & - & 0.629 & - \\
    % \quad +\Algname & 0.259 & \textcolor{teal}{0.008} & 0.008 & \textcolor{teal}{0.001} & 109.77 & \textcolor{teal}{7.53} & 0.579 & \textcolor{red}{0.007} & 0.279 & \textcolor{red}{0.073} & 0.344 & \textcolor{teal}{0.068} & 4.47 & \textcolor{teal}{8.64} & 0.669 & \textcolor{teal}{0.040}  \\
    % \midrule
    % GPT-4o & 0.521 & - & 0.079 & - & 40.87 & - & 0.797 & - & 0.496 & - & 0.583 & - & 3.67 & - & 0.881 & - \\
    % \quad +\Algname & 0.509 & \textcolor{red}{0.012} & 0.088 & \textcolor{teal}{0.009} & 41.68 & \textcolor{teal}{0.081} & 0.783 & \textcolor{red}{0.014} & 0.498 & \textcolor{teal}{0.002} & 0.571 & \textcolor{red}{0.012} & 1.57 & \textcolor{teal}{2.10} & 0.846 & \textcolor{red}{0.035} \\
    \bottomrule[1.25pt]
    \end{tabular}
    }
    % \vspace{-0.25in}
\end{table*}
